How Transferable are the Representations Learned by Deep Q Agents?

In this paper, we consider the source of Deep Reinforcement Learning (DRL)'s sample complexity, asking how much derives from the requirement of learning useful representations of environment states and how much is due to the sample complexity of learning a policy. While for DRL agents, the distinction between representation and policy may not be clear, we seek new insight through a set of transfer learning experiments. In each experiment, we retain some fraction of layers trained on either the same game or a related game, comparing the benefits of transfer learning to learning a policy from scratch. Interestingly, we find that benefits due to transfer are highly variable in general and non-symmetric across pairs of tasks. Our experiments suggest that perhaps transfer from simpler environments can boost performance on more complex downstream tasks and that the requirements of learning a useful representation can range from negligible to the majority of the sample complexity, based on the environment. Furthermore, we find that fine-tuning generally outperforms training with the transferred layers frozen, confirming an insight first noted in the classification setting.

==> sections/Notes.tex <==
\section{Notes}

\begin{enumerate}
    \item \textbf{This analysis is wrong, but the results were still observed, why?}  Learning rate makes a big difference - training a game from scratch, changing only the horizon from 2M to 5M to 50M results in 3 very different agents, even with respect to the time step.  I am pretty sure the only difference is that the learning rate decays over time with respect to the horizon, therefore the longer the horizon, the more exploration that can be done.  
    \item selected games: \textbf{}
    \begin{enumerate}
        \item riverraid [scrolling shooter]
        \item berzerk [platform]
        \item krull [fighting]
        \item (bonus) robotank [shooter]
    \end{enumerate}
    \item Experiments:
    \begin{enumerate}
        \item \textit{Fill from scripts here to keep track of what has been ran}
    \end{enumerate}
\end{enumerate}

%==========================================================================
\section{Confusion}

Point number 1 in the above section may be wrong.  

looked at the paper again - it is the value of epsilon greedy in the epsilon greedy exploration that changes with respect to the time step - this is not needed in rainbow as they use noisy weights for exploration.  

